Learning Variational Word Masks to Improve the Interpretability of Neural Text Classifiers

To build an interpretable neural text classifier, most of the prior work has focused on designing inherently interpretable models or finding faithful explanations. A new line of work on improving model interpretability has just started, and many existing methods require either prior information or human annotations as additional inputs in training. To address this limitation, we propose the variational word mask (VMASK) method to automatically learn task-specific important words and reduce irrelevant information on classification, which ultimately improves the interpretability of model predictions. The proposed method is evaluated with three neural text classifiers (CNN, LSTM, and BERT) on seven benchmark text classification datasets. Experiments show the effectiveness of VMASK in improving both model prediction accuracy and interpretability.

==> app2.tex <==
\section{Proof}
\label{sec:proof}

\yfcomment{part of this section can be used to replace the end of section 3.1 and the whole section 3.2.}

Recall the three random variables defined in our model
\begin{itemize}
\item $\vec{Y}$: one-hot random vector as class label indicator
\item $\vec{X} = (X_1,\dots, X_T)$: a sentence with $T$ words, where each $X_t$ is a word index
\item $\vec{Z} = (Z_1,\dots, Z_T)$: a sequence of random variables, where the sample space of each $Z_t$ is defined as $Z_1\in\{0, x_t\}$ and $x_t$ is the corresponding word index value.
\end{itemize}

Assume $q(X,Y,Z)$ is the probability distribution that we are used to approximate the true distribution of these three random variables, $p(X,Y,Z)$.
Following the standard practice in the Information Bottleneck theory, we assume the dependency relation among the three random varibales is specified by the following Markov chain
\begin{equation}
  \label{eq:markov}
  \vec{Y} \leftrightarrow \vec{X} \leftrightarrow \vec{Z}
\end{equation}
and the corresponding Information Bottleneck function is defined as
\begin{equation}
  \label{eq:ib}
  I(\vec{Z},\vec{Y}) - \beta\cdot I(\vec{Z},\vec{X})
\end{equation}
where $I(\cdot,\cdot)$ is the mutual information and $\beta\in\mathbb{R}_{+}$ is a coefficient to balance the two mutual information items.
The objective is to learn $\vec{Z}$ that can do a good job on predicting $\vec{Y}$ but has minimal mutual information with $\vec{X}$.

In this section, we will start from \autoref{eq:ib} and provide a justification of the objective function in \todo{add equation index} in \autoref{sec:method}.
The following derivation is similar to the variational information bottleneck, where the difference is that our starting point is the approximation distribution $q(\vec{X},\vec{Y},\vec{Z})$ instead of the true distribution $p(\vec{X},\vec{Y},\vec{Z})$.

Recall the definition of $I(\vec{Z},\vec{Y})$ under the distribution of $p(\vec{Z},\vec{Y})$, we have \footnote{For notation convenience, let us assume all three random variables are continuous for now.}
\begin{eqnarray}
  I(\vec{Z},\vec{Y})
  &=& \int d\vec{y} d\vec{z} q(\vec{y},\vec{z})\log \frac{q(\vec{y},\vec{z})}{q(\vec{y})q(\vec{z})}\\
  &=& \int d\vec{y} d\vec{z} q(\vec{y},\vec{z})\log \frac{q(\vec{y}|\vec{z})}{q(\vec{y})}\\
  &=& \int d\vec{y}d\vec{z} q(\vec{y},\vec{z}) \log q(\vec{y}|\vec{z})\nonumber\\
  & & + H_q(\vec{Y})
\end{eqnarray}

Now, if we replace $\log q(\vec{y}|\vec{z})$ with the conditional probability derived from the true distribution $\log p(\vec{y}|\vec{z})$, we have
\begin{equation}
\begin{aligned}
\label{eq:L_bound}
& \sum_{\vec{y}} \sum_{\vec{z}} q(\vec{y},\vec{z})\log q(\vec{y}|\vec{z}) \\
&= \sum_{\vec{y}} \sum_{\vec{z}} q(\vec{y},\vec{z})\log \frac{q(\vec{y}|\vec{z})p(\vec{y}|\vec{z})}{p(\vec{y}|\vec{z})} \\
&=\sum_{\vec{y}} \sum_{\vec{z}} q(\vec{y},\vec{z})\log p(\vec{y}|\vec{z}) + \kldist{q(\vec{y}|\vec{z})}{p(\vec{y}|\vec{z})} \\
&\geq \sum_{\vec{y}} \sum_{\vec{z}} q(\vec{y},\vec{z})\log p(\vec{y}|\vec{z})
\end{aligned}
\end{equation}

\begin{equation}
  \int d\vec{y} d\vec{z}  q(\vec{y},\vec{z})\log q(\vec{y}|\vec{z}) \geq \int d\vec{y} d\vec{z}  q(\vec{y},\vec{z})\log p(\vec{y}|\vec{z})
\end{equation}
Therefore,
\begin{eqnarray}
  \label{eq:izy-lower}
  I(\vec{Z},\vec{Y})
  &\geq& \int d\vec{y}d\vec{z} q(\vec{y},\vec{z}) \log p(\vec{y}|\vec{z}) + H_q(\vec{Y})\\
  &=& \int d\vec{x} d\vec{y} d\vec{z} q(\vec{x},\vec{y},\vec{z})\log p(\vec{y}|\vec{z})\nonumber\\
  & & + H_q(\vec{Y})\\
  &=& \int d\vec{x} d\vec{y} d\vec{z} q(\vec{x}) q(\vec{y}|\vec{x}) q(\vec{z}|\vec{x}) \log p(\vec{y}|\vec{z})\nonumber\\
  & & + H_q(\vec{Y})
\end{eqnarray}
the last step uses $q(\vec{x},\vec{y},\vec{z}) = q(\vec{x})q(\vec{y}|\vec{x}) q(\vec{z}|\vec{x})$, which is a factorization based on the Markov chain.

Since $q(\vec{X},\vec{Y},\vec{Z})$ is the approximation defined by ourselves, given a specific observation $(\vec{x}^{(i)},\vec{y}^{(i)})$, the empirical distribution $q(\vec{X}^{(i)},\vec{Y}^{(i)})$ is simply defined as a multiplication of two Delta functions
\begin{equation}
  q(\vec{X}^{(i)}=\vec{x},\vec{Y}^{(i)}=\vec{y}) = \delta_{\vec{x}^{(i)}}(\vec{x})\cdot\delta_{\vec{y}^{(i)}}(\vec{y}).
\end{equation}

Then, \autoref{eq:izy-lower} with $\vec{X}^{(i)}$ and $\vec{Y}^{(i)}$ can be further simplified as
\begin{eqnarray}
  \label{eq:vib-1}
  I(\vec{Z},\vec{Y}^{(i)})
  &\geq& \int d\vec{z} q(\vec{z}|\vec{x}^{(i)}) \log p(\vec{y}^{(i)}|\vec{z})\\
  &=& \expect{\log p(\vec{y}^{(i)}|\vec{z})}{q(\vec{z}|\vec{x}^{(i)})}
\end{eqnarray}

Now, let us consider the mutual information $I(\vec{Z},\vec{X})$
\begin{eqnarray}
  I(\vec{Z},\vec{X})
  &=& \int d\vec{x} d\vec{z} q(\vec{x},\vec{z})\log \frac{q(\vec{x},\vec{z})}{q(\vec{x}) q(\vec{z})}\\
  &=& \int d\vec{x} d\vec{z} q(\vec{x},\vec{z})\log \frac{q(\vec{z}|\vec{x})}{q(\vec{z})}\\
  &=& \int d\vec{x} d\vec{z} q(\vec{x},\vec{z})\log q(\vec{z}|\vec{x})\nonumber\\
  & & - \int d\vec{x} d\vec{z} q(\vec{x},\vec{z})\log q(\vec{z})
\end{eqnarray}

By replacing $q(\vec{Z})$ with a prior distribution of $\vec{z}$, $p_0(\vec{z})$, we have
\begin{equation}
  \int d\vec{x} d\vec{z} q(\vec{x},\vec{z})\log q(\vec{z}) \geq
  \int d\vec{x} d\vec{z} q(\vec{x},\vec{z})\log p_0(\vec{z}).
\end{equation}
Therefore,
\begin{eqnarray}
  \label{eq:vib-2}
  I(\vec{Z},\vec{X})
  &\leq& \int d\vec{x} d\vec{z} q(\vec{x},\vec{z})\log q(\vec{z}|\vec{x})\nonumber\\
  & & - \int d\vec{x} d\vec{z} q(\vec{x},\vec{z})\log p_0(\vec{z})\\
  &=& \int d\vec{x} q(\vec{x})\kldist{q(\vec{z}|\vec{x})}{p_0(\vec{z})}\\
  &=&  \expect{\kldist{q(\vec{z}|\vec{x})}{p_0(\vec{z})}}{q(\vec{x})}
\end{eqnarray}

Given $(\vec{x}^{(i)},\vec{y}^{(i)})$, Substituting \autoref{eq:vib-1} and \autoref{eq:vib-2} into \autoref{eq:ib} gives us a lower bound of the informaiton bottleneck 
\begin{equation}
  \label{eq:ib-obj-1}
  \begin{split}
    I(\vec{Z},\vec{Y})
    &- \beta\cdot I(\vec{Z},\vec{X})\\
    &\geq \expect{\log p(\vec{y}^{(i)}|\vec{z})}{q(\vec{z}|\vec{x}^{(i)})}\\
    & ~~~-\beta\expect{\kldist{q(\vec{z}|\vec{x})}{p_0(\vec{z})}}{q(\vec{x})}\\
    &= \mathcal{L}
  \end{split}
\end{equation}
The learning objective is to maximize \autoref{eq:ib-obj-1} with respect to the approximation distribution $q(\vec{X},\vec{Y},\vec{Z})$.
As $\vec{X}$ and $\vec{Y}$ are both observed in our problem, the only one left in the approximation distribution is $q(\vec{Z}|\vec{X})$.
Similarly to the objective function in variational inference, the first term in $\mathcal{L}$ is to make sure the information in $q(\vec{Z}|\vec{X})$ for predicting $\vec{Y}$, while the second term in $\mathcal{L}$ is to regularize $q(\vec{Z}|\vec{X})$ with a predefined prior distribution $p_0(\vec{Z})$.

The last step of verifying our objective function is to notice that, given $X_t^{(i)}=x_t^{(i)}$ every $Z_t$ can be redefined as
\begin{equation}
  Z_t = x_t^{(i)}\cdot R_t
\end{equation}
where $R_t\in\{0,1\}$ is a standard Bernoulli distribution. Then, $\vec{Z}$ can be reparameterized as $\vec{Z}=\vec{R}\circ\vec{x}^{(i)}$ with $\vec{R}=(R_1,\dots, R_T)$.
The lower bound $\mathcal{L}$ can be rewritten with the random variable $\vec{R}$ as
\begin{equation}
  \label{eq:ib-obj}
  \begin{split}
    \mathcal{L}
    = &  \expect{\log p(\vec{y}^{(i)}|\vec{r},\vec{x}^{(i)})}{q(\vec{r}|\vec{x}^{(i)})}\\
    & ~~~-\beta\cdot \kldist{q(\vec{r}|\vec{x}^{(i)})}{p_0(\vec{r})}
  \end{split}
\end{equation}



==> method_old.tex <==
\section{Method}
\label{sec:method}

\subsection{Variational Information Bottleneck}
\label{subsec:vib}
Let $X$ represent the input variable which contains a set of sentences, and $Y$ represent the corresponding output variable such as the prediction label in text classification. For an input text $\vec{x}=[\vec{x}_{1}^{T}, \vec{x}_{2}^{T}, \cdots, \vec{x}_{T}^{T}]^{T}$, $\vec{x}_{i}\in \mathbb{R}^{d}$ denotes the embedding of the i-th word. To train a good model, we basically aim to find a map $f(\cdot)$ between the input-output pairs $(X, Y)$, which minimizes the loss function with respect to $Y$ and the ground-truth variable $Y_{t}$.
\begin{equation}
\label{eq:basic_obj_func}
\min_{f} \mathcal{L}(Y_{t}; Y),
\end{equation}
where $Y=f(X)$, and $\mathcal{L}$ is the cross-entropy loss. 


Although a deep neural network can easily achieve a high accuracy on training data, it tends to be overfitting, harming generalization to test data. Let $V$ represent the vocabulary built on the training set. Our goal is to learn a global mask $M\in \mathbb{R}^{N\times C}$ to restrict the information of each token in the vocab for a specific task, where $N$ is the number of tokens in the vocabulary and $C$ is the number of output categories. We insert the information bottleneck (IB) into the original model (after the embedding layer), and train the model and IB jointly by minimizing
\begin{equation}
\begin{aligned}
\label{eq:mask_obj_func}
\mathcal{L}_{loss} &=\mathcal{L}_{cross-entropy} + \beta \mathcal{L}_{information} \\
&=\mathcal{L}(Y_{t}; Y') + \beta I(X, X'), 
\end{aligned}
\end{equation}
where $X'=M(X)$, $Y'=f(X')$, $I(\cdot ; \cdot)$ is mutual information, and $\beta$ coordinates the prediction performance and the information kept in $X'$. Note that the mask learns to keep the information associated with ground-truth label, which makes the loss function \autoref{eq:mask_obj_func} different from the traditional IB loss function which is $\mathcal{L}_{IB}=-I(Y, X')+I(X, X')$. $\mathcal{L}_{IB}$ is to keep as little information from $X$, while retain the same prediction $Y$.


The mutual information between $X$ and $X'$ can be formulated as
\begin{equation}
\begin{aligned}
\label{eq:mutual_infor}
I(X, X') &= \mathbb{E}_{X, X'}\left[\log\frac{p(X, X')}{p(X)p(X')}\right] \\
&=\mathbb{E}_{X}\left[\mathbb{E}_{X'\sim p(X'|X)}\left[\log \dfrac{p(X'|X)}{p(X')}\right]\right].
\end{aligned}
\end{equation}
As the estimations of the two distributions $p(X'|X)$ and $p(X')$ are intractable, we resort to variational IB to obtain the upper bound of the mutual information. A variational distribution $q(X'|X)$ is introduced, and the mutual information can be rewritten as
\begin{equation}
\label{eq:var_mutual_infor}
I(X, X')=\mathcal{L}_{upper}-\mathbb{E}_{X}\left[KL\left[q(X'|X)\|p(X'|X)\right]\right],
\end{equation}
where $\mathcal{L}_{upper}=\mathbb{E}_{X}\left[KL\left[q(X'|X)\|p(X')\right]\right]$, and $KL[\cdot\|\cdot]$ is the KL-divergence between two distributions. As the second term on the right side is a KL divergence and hence non-negative, we have $I(X, X')\leq\mathcal{L}_{upper}$.


There are two possible methods to compute the mutual information.

\paragraph{Global Masks.} For an input $\vec{x}$, IB is applied on the word embedding of each word $\vec{x}_{i}$ individually. A common way to restrict the information is to add noise.
\begin{equation}
\label{eq:add_noise}
\vec{x}_{i}'=\lambda_{i} \vec{x}_{i}+(1-\lambda_{i})\vec{\epsilon},
\end{equation}
where $\vec{\epsilon}\sim\mathcal{N}(\vec{\mu}_{\vec{x}_{i}}, \Sigma_{\vec{x}_{i}})$, and $\lambda_{i}\in[0, 1]$ controls the discarded information and injected noise. We further estimate a mask vector $M_{i}=[\lambda_{i, 1}, \lambda_{i, 2},\cdots, \lambda_{i, C}]^T$ for each token in the vocab, where $\lambda_{i, c}$ corresponds to category $c\in C$. During training, $\vec{x}_{i}$ multiplies each value in the mask vector separately, that is $\vec{x}_{i, c}'=\lambda_{i, c} \vec{x}_{i}+(1-\lambda_{i, c})\vec{\epsilon}$, and then $\{\vec{x}_{i, 1}', \vec{x}_{i, 2}', \cdots, \vec{x}_{i, C}'\}$ go through the model in parallel. At the output layer, $y'=\arg\max\limits_{c\in C}\{f(\vec{x}_{i, 1}')_{1}, f(\vec{x}_{i, 2}')_{2}, \cdots, f(\vec{x}_{i, C}')_{C}\}$. For $\mathcal{L}_{upper}(\vec{x})$, we average the mutual information of words in a sentence over all categories, $\mathcal{L}_{upper}(\vec{x})\leq\frac{1}{TC}\sum\limits_{c\in C}\sum\limits_{i\in T}KL\left[q(\vec{x}_{i, c}'|\vec{x}_{i})\|h(\vec{x}_{i, c}')\right]$, where $h(\vec{x}_{i, c}')$ is also a variational distribution to $p(\vec{x}_{i, c}')$. We usually assume that $h(\vec{x}_{i, c}')\sim\mathcal{N}(\vec{\mu}_{\vec{x}_{i}}, \Sigma_{\vec{x}_{i}})$ and $q(\vec{x}_{i, c}'|\vec{x}_{i})$ is also Gaussian-distributed.

But the problem is that we do not know the mean and variance of $\vec{x}_{i}$, which causes some difficulty in calculating $\mathcal{L}_{upper}$. Actually, I have no idea about how to estimate the empirical mean and variance of $\vec{x}_{i}$.

\paragraph{Variational IB.} As the true posterior $p_{\theta}(\vec{x}_{i}'|\vec{x}_{i})$ is intractable, another way is to use a variational approximate posterior $q_{\phi}(\vec{x}_{i}'|\vec{x}_{i})$ which is Gaussian-distributed with mean and diagonal covariance obtained from $\vec{x}_{i}$ with a feedforward neural network $M_{\phi}(\cdot)$. $h_{\xi}(\vec{x}_{i}')$ is also a Gaussian distribution, and its mean and covariance will be learned during training. As $\vec{x}_{i}' \in \mathbb{R}^{d}$ has the same dimension as $\vec{x}_{i}$, the output of $M_{\phi}(\cdot)$ has 2d dimension, where the first d variables form the mean vector of $q_{\phi}(\vec{x}_{i}'|\vec{x}_{i})$ and the latter d variables are the diagonal elements of the covariance matrix. With the two Gaussian distributions, the KL-divergence can be easily calculated. The output of mask is a matrix $\vec{x}'=[\vec{x}_{1}'^{T}, \vec{x}_{2}'^{T}, \cdots, \vec{x}_{T}'^{T}]^{T}$ which will be further input to the model for prediction.


The final optimization function is:
\begin{equation}
\label{eq:final_obj_func}
\min_{f, \phi, \xi} \mathbb{E}_{\vec{x}, y_{t}}\left[\mathbb{E}_{\vec{x}_{i}'\sim q_{\phi}(\vec{x}_{i}'|\vec{x}_{i})}\left[\mathcal{L}(y_{t}; f(\vec{x}_{i}'))\right]\right]+\beta\mathcal{L}_{upper},
\end{equation}
where $\mathcal{L}_{upper}=\mathbb{E}_{\vec{x}}\left[ KL\left[q_{\phi}(\vec{x}_{i}'|\vec{x}_{i})\|h_{\xi}(\vec{x}_{i}')\right]\right]$. Note that for back-propagation, "reparameterization trick" should be applied to generate $\vec{x}'$.

$\vec{x}_{i}'\in \mathbb{R}^{d'}$ can has lower and more compress dimension than $\vec{x}_{i}$.

\subsection{Variational Mask}
\label{subsec:vmask}
We learn a variational mask $r_i$ for each word embedding $\vec{x}_{i}$, and multiply them to generate a post-embedding $\vec{x}_{i}'=r_{i}\vec{x}_{i}$. We assume the prior $p(r)\sim Beta(\alpha_{0}, \beta_{0}), \alpha_{0}=\beta_{0}=0.5$. The intuition is that $r_i$ sampled from the posterior $p(r_{i}|\vec{x}_{i})$ can be close to 0 or 1 with a high probability, so that it can help identify some important or unimportant words for a specific task. As each $r_i$ is multiplied with each word $\vec{x}_{i}$ individually, we have $p_{\theta}(r|x)=\prod\limits_{i\in T}p_{\theta}(r_i|\vec{x}_{i})$.

The loss function contains two components,
\begin{equation}
\label{eq:new_loss_func}
\mathcal{L}_{loss} =\mathcal{L}_{cross-entropy} + \gamma\mathbb{E}_{\vec{x}}\left[ KL\left[p_{\theta}(r_i|\vec{x}_{i})\|p_{\theta}(r_i)\right]\right].
\end{equation}
We utilize variational distribution again to compute the upper bound of the second term,

\begin{small}
\begin{equation}
\label{eq:upper_bound}
\mathbb{E}_{\vec{x}}\left[ KL\left[p_{\theta}(r_i|\vec{x}_{i})\|p_{\theta}(r_i)\right]\right]\leq \mathbb{E}_{\vec{x}}\left[ KL\left[q_{\phi}(r_i|\vec{x}_{i})\|p_{\theta}(r_i)\right]\right],
\end{equation}
\end{small}%
where $q_{\phi}(r_i|\vec{x}_{i})\sim Beta(\alpha_i, \beta_i)$ with $\alpha_i$ and $\beta_i$ obtained from $\vec{x}_{i}$ with a feedforward neural network $M_{\phi}(\cdot)$. The output of $M_{\phi}(\cdot)$ has two dimensions, where the first one is $\alpha_i$ and the second one is $\beta_i$. Note that to guarantee the values of $\alpha_i$ and $\beta_i$ are positive, we take the square of the output and add a small positive value (1e-8). For the two Beta distributions, we can directly calculate the KL-divergence\footnote{\url{https://pytorch.org/docs/stable/distributions.html\#module-torch.distributions.kl}{}}. During training, we utilize the reparameterization trick\footnote{\url{https://pytorch.org/docs/stable/distributions.html}{}} in pytorch for back-propagation.
